GRAPHEVAL: Quantifying Reasoning Uncertainty to Assess Trustworthiness in LLMs

Unfaithful reasoning undermines the trustworthiness of Large-Language Models. In mission-critical settings where reasoning errors can lead to catastrophic physical, financial, or legal consequences, accuracy without faithfulness is insufficient. Decoding methods such as Self-Consistency (SC) may fail to detect these failures because they evaluate final-answer agreement while ignoring the reasoning that produces it. We therefore investigate whether reasoning uncertainty can be reliably quantified, used to select more faithful answers, and evaluated under adversarial conditions. To address these questions, we introduce GRAPHEVAL, a framework that estimates reasoning uncertainty to assess models' trustworthiness and shift evaluation from final-answer consensus to the semantic and causal consistency of the reasoning that produces it. We propose a novel uncertainty quantification metric based on the Graph Reasoning Coherence Score (GRCS), where lower coherence reflects higher reasoning uncertainty. The resulting uncertainty increases as reasoning faithfulness decreases in 88.9% of evaluated configurations and outperforms SOTA baselines in 77.8% of comparisons, while being, on average, 32.5x faster. For decoding, we introduce Graph Self Consistency (GSC), which accounts for within-answer reasoning uncertainty, ignored by SC, and selects the more logically sound answer in 24.9% more SC-GSC disagreements. Finally, under adversarial ablation, we show that removing GSC-selected paths degrades faithfulness in up to 55% of answers (average: 30.59%), with drops exceeding 50% in some settings.

==> pic/attack_ablation.tex <==
% %\begin{figure}
% \begin{wrapfigure}[19]{r}{0.7\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]%\includegraphics[scale=0.25]
%     {pic/ablation_degradation_bars.pdf} 
%     \caption{\textbf{Adversarial Medoid Ablation}. (Left: StrategyQA, Right: MedQA). 
%     %\textit{Methodology}: We forced models to answer questions where GSC achieved 100\% accuracy, and SC achieved 0\%, but strictly banned them from using their original winning logic (the Medoid CoT selected by GSC). 
%    %\textit{Results}: 
%    Straying from the primary reasoning path exposes severe structural fragility. Models typically suffer massive drops in accuracy and faithfulness, or resort to unfaithful ``lucky guesses'' (\eg, DeepSeek on MedQA). While models occasionally find a valid backup path, their performance becomes highly volatile and unpredictable. This confirms the Medoid is the most important path for reliable deduction.}
%     \label{fig:medoid_ablation_fig}
% %\end{figure}
% \end{wrapfigure}

%%%% DP: Needs updated table %%%%

\begin{figure}
    \begin{minipage}{0.55\textwidth}
    \begin{subfigure}[b]{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{pic/target_attack_table.pdf}
    \end{subfigure}
    \end{minipage}
    \begin{minipage}{0.45\textwidth}
            \caption{\textbf{Adversarial Medoid Ablation}. Deviating from %the primary reasoning path, or 
            medoid causes models to suffer from severe structural fragility, resulting in significant accuracy loss and unpredictable, unfaithful performance. This instability confirms that the Medoid path is the essential foundation for maintaining reliable and consistent deduction. \dpal{UPDATE}}
    \label{fig:medoid_ablation_fig}
    \end{minipage}
    \vspace{-6mm}
\end{figure}


\begin{comment}
\begin{figure}
    \begin{minipage}{0.55\textwidth}
        \begin{subfigure}[b]{\linewidth}
            \centering
            \includegraphics[width=0.5\linewidth]{pic/ablation_degradation_strategyqa.pdf}
        \end{subfigure}
    \end{minipage}
    \hfill
    \begin{minipage}{0.55\textwidth}
        \begin{subfigure}[b]{\linewidth}
            \centering
            \includegraphics[width=0.5\linewidth]{pic/ablation_degradation_gpqa.pdf}
        \end{subfigure}
    \end{minipage}
    \begin{minipage}{\textwidth}
        \caption{\textbf{Adversarial Medoid Ablation}. Deviating from %the primary reasoning path, or 
        medoid causes models to suffer from severe structural fragility, resulting in significant accuracy loss and unpredictable, unfaithful performance. This instability confirms that the Medoid path is the essential foundation for maintaining reliable and consistent deduction.}
        \label{fig:medoid_ablation_fig}
    \end{minipage}
    \vspace{-6mm}
\end{figure}
\end{comment}

==> pic/broad_attack.tex <==
%\begin{figure}[h]
%\begin{wrapfigure}{r}{0.85\textwidth}
\setlength{\intextsep}{0pt} % Default is usually larger
%\begin{wrapfigure}[15]{r}{0.7\textwidth}
%    \centering
%    \vspace{-10pt}
%    \includegraphics[width=\linewidth]
    %\includegraphics[scale=0.26]
%    {pic/scatter_strategyqa.pdf} 
%    \caption{\textbf{Population-Level %Medoid 
%    Ablation for StrategyQA}. 
    %\textit{Methodology}: 
    %For each question and model, we ablate the GSC medoid by forbidding its logic, sample $K=5$ alternative CoTs at $T=0.7$, and compare per-question adversarial accuracy and faithfulness against the original baseline.
    %\textit{Results}: 
    %For each question, we ablate the GSC-selected medoid by forbidding its logic, sample $K=20$ alternative CoTs, and plot the change in adversarial accuracy ($\Delta$Accuracy) against the change in reasoning fidelity ($\Delta$Faithfulness).
%    Medoid ablation often leaves %nominal 
%    accuracy unchanged ($\Delta\text{Accuracy}=0$) while degrading faithfulness for %across 
%    all GLLMs. In smaller GLLMs, high %significant 
%    negative correlations %further 
%    show that %apparent 
%    accuracy gains %($\Delta\text{Accuracy}>0$) 
%    often reflect unfaithful ``lucky guesses'' rather than valid recovery. %\textit{(Horizontal jitter applied for visualization; regressions use exact data).} 
%    } %while the baselines remain weak.}
%    \label{fig:broad_ablation_fig}
    %\vspace{-5mm}
%\end{figure}
%\end{wrapfigure}

\setlength{\intextsep}{0pt} % Default is usually larger

\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{pic/scatter_strategyqa.pdf}
    \caption{\textbf{Population-Level Ablation for StrategyQA}. 
    Medoid ablation often leaves accuracy unchanged ($\Delta\text{Accuracy}=0$) while degrading faithfulness for all GLLMs. In smaller GLLMs, high negative correlations show that accuracy gains often reflect unfaithful ``lucky guesses'' rather than valid recovery.}
    \label{fig:broad_ablation_fig}
\end{figure}

==> pic/complexitygraph.tex <==
\begin{figure}[h]
    \centering
    \begin{tikzpicture}[scale=0.6]
        \begin{axis}[
            xlabel={\textbf{Maximum node count ($m$)}},
            ylabel={\textbf{Computational Operations (log scale)}},
            domain=1:10,
            samples=200,
            legend pos=north west,
            grid=both,
            grid style={line width=.1pt, draw=gray!10},
            major grid style={line width=.2pt, draw=gray!50},
            ymode=log,
            restrict y to domain=1:1e15,
            xmin=1, xmax=10,
            ymin=1,
            width=0.75\linewidth,
            % --- thick axes ---
            axis line style={line width=2pt},
            % --- bold tick labels ---
            tick label style={font=\bfseries, line width=2pt},
            % --- bold axis labels ---
            label style={font=\bfseries},
            yticklabel style={font=\bfseries, /pgf/number format/assume math mode=true},
        ]
        % Cubic complexity (your approach)
        \addplot[blue, line width=4pt] {x^3};
        \addlegendentry{Bipartite Matching $\mathcal{O}(m^3)$}
        % Exponential complexity (exact GED) — m^m approximation
        \addplot[red, line width=4pt, dashed] {x^x};
        \addlegendentry{GED $\mathcal{O}(m^m)$}
        \end{axis}
    \end{tikzpicture}
    \caption{Worst-case theoretical time complexity comparison between GED ($\mathcal{O}(m^m)$) and the bipartite matching approximation ($\mathcal{O}(m^3)$) used in our approach, as a function of the maximum node count $m$.}
    \label{fig:complexity_comparison}
\end{figure}

==> pic/discard_rate.tex <==
% pic/uq_analysis_minipage.tex
% Modular minipage structure for side-by-side Delta comparison charts.
% Compatible with IEEEtran and other major journal templates.

\begin{figure*}[t]
    \centering
    
    % Left Column: GRCS vs. CoTA
    \begin{minipage}{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{pic/entropy_retention_chart_gsm8k.pdf}
        \vspace{-2mm}
        \centerline{\small\textbf{(a) GSC Discard Rate on GSM8K}}
    \end{minipage}
    \hfill
    % Right Column: GRCS vs. Topo-UQ
    \begin{minipage}{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{pic/entropy_retention_chart_medqa.pdf}
        \vspace{-2mm}
        \centerline{\small\textbf{(b) GSC Discard Rate on MedQA}}
    \end{minipage}
    
    \caption{\textbf{GSC Discard Rate vs SC} 
    We divide all reasoning paths, and their answers, into conditional entropy quartiles (Q1: low entropy; Q4: high entropy). On smaller GLLMs, GSC discards a high percentage of paths where entropy is the highest (Q4), because they are related to higher uncertainty. With more capable GLLMs, GSC retains almost all reasoning paths.}
    \label{fig:entropy_retention_charts}
    \vspace{-4mm}
\end{figure*}

==> pic/exp2_res.tex <==
%\begin{figure}[h]
\begin{wrapfigure}[20]{r}{0.7\textwidth}
    \centering
    \includegraphics[width=\linewidth]{pic/uq_bars_PCC_exp2.pdf}
    %\includegraphics[scale=0.16]{pic/uq_bars_PCC_exp2.pdf} 
    \caption{\textbf{UQ Analysis across increasing complexities}. 
    \textit{Methodology}: Following the methodology of \Cref{fig:gsm8k_res}, we report PCC for Dispersion, Entropy, and GRCS across three LLMs and four datasets of increasing difficulty.
    \textit{Results}: 1) Dispersion and Entropy are unstable, often yielding positive correlations (e.g., LLaMA 3.1 8B and Phi-4 on GSM8K and MedQA). 2) GRCS, instead, stays negative in nearly all settings, making it the most reliable signal of unfaithful reasoning. 3) Its advantage persists even on harder domains like MedQA, where it falls below $-0.2$ for both LLaMA 3.1 8B and Phi-4. } %while the baselines remain weak.}
    \label{fig:exp2_fig}
    %\vspace{-5mm}
%\end{figure}
\end{wrapfigure}

==> pic/gsc_scores_epistaxis.tex <==
\begin{figure}[h]
%\begin{wrapfigure}{r}{0.85\textwidth}
    \centering
    %\includegraphics[width=\linewidth]
    \includegraphics[scale=0.22]{pic/case_gsc_medqa_epistaxis.pdf} 
    \caption{\textbf{Combined medoid objective across the 20 Phi-4 CoTs for MedQA question 440.}
    The medoid (CoT~13) is the unique top-ranked trace, while most of the next highest-scoring CoTs are incorrect. Thus, GSC recovers the correct answer in a difficult regime where the reasoning pool is dominated by high-scoring but misordered clinical traces.}
    \label{fig:gsc_scores_epistaxis_fig_appendix}
    \vspace{5mm}
\end{figure}
%\end{wrapfigure}

==> pic/gsc_scores_iphone.tex <==
\begin{figure}[h]
%\begin{wrapfigure}{r}{0.85\textwidth}
    \centering
    %\includegraphics[width=\linewidth]
    \includegraphics[scale=0.22]{pic/case_gsc_iphone_strategyqa.pdf} 
    \caption{\textbf{Combined medoid objective across the 20 GLLM-generated CoTs for the lolcats/iPhone StrategyQA example.}
    %\textit{Results}: The figure shows that the top of the ranking is dominated by coherent reasoning traces, indicating that the faithful solution pattern forms the most stable and reproducible cluster in the sample. In contrast, incoherent or hallucinated traces are more dispersed and generally receive weaker scores. This makes clear why GSC succeeds: rather than following surface-level answer frequency, it selects the structurally central reasoning path supported by the most coherent neighborhood.}
    The GSC selected medoid CoT, having the highest GSC Score, is CoT 05. The highest-ranked traces form a coherent cluster, while hallucinated traces are more dispersed and score lower. Thus, GSC succeeds by selecting the structurally central path rather than the most frequent answer.}
    \label{fig:gsc_scores_iphone_fig_appendix}
    %\vspace{-5mm}
\end{figure}
%\end{wrapfigure}

==> pic/gsc_scores_jindall.tex <==
\begin{figure}[h]
%\begin{wrapfigure}{r}{0.85\textwidth}
    \centering
    %\includegraphics[width=\linewidth]
    \includegraphics[scale=0.22]{pic/case_gsc_jindall.pdf} 
    \caption{\textbf{Combined medoid objective across the 20 GLLM-generated CoTs for the Bobby Jindal StrategyQA example.}
    \textit{Methodology}: Each CoT is converted into a reasoning graph and scored by the main paper’s medoid objective, which combines normalized graph centrality and path consensus. Bars are sorted by this score; green denotes correct (\emph{true}) CoTs, red denotes incorrect (\emph{false}) CoTs, and hatching marks the GSC-selected medoid.
    %\textit{Results}: The figure makes the selection mechanism visually explicit. The highest-scoring region is dominated by correct \emph{true} traces, which form a dense and internally consistent cluster; the selected medoid lies within this region. By contrast, most incorrect \emph{false} traces receive lower scores, reflecting their fragmented and weakly supported reasoning patterns. Thus, although standard SC follows the numerical \emph{false} majority, GSC correctly selects the coherent \emph{true} minority because it is collectively better supported in semantic and structural space.}
    \textit{Results}: The figure makes the selection mechanism explicit. High-scoring traces cluster around the correct \emph{true} reasoning paths, with the medoid located within this dense and semantically consistent region. In contrast, most incorrect \emph{false} traces receive lower scores, reflecting weaker structural and semantic support. Consequently, while standard SC follows the numerical \emph{false} majority, GSC selects the coherent \emph{true} minority.}
    \label{fig:gsc_scores_jindall_fig_appendix}
    %\vspace{-5mm}
\end{figure}
%\end{wrapfigure}

==> pic/gsm8k_correlations.tex <==
%\begin{figure}
\setlength{\intextsep}{0pt} % Default is usually larger

\begin{wrapfigure}[16]{r}{0.7\textwidth}
    \centering
    %\includegraphics[width=\linewidth]
    \includegraphics[width=\linewidth]    {pic/uq_bars_PCC.pdf} 
    \caption{\textbf{Uncertainty Qunatification Analysis}. 
    %\textit{Methodology}: We measure how well different uncertainty metrics correlate with actual reasoning Faithfulness across three LLMs on GSM8K dataset, reporting Pearson (PCC), Spearman (SRC) and Kendall (KRC) correlations. A reliable uncertainty metric must show a strong negative correlation with Faithfulness. 
    %\textit{Methodology}: We correlate uncertainty with reasoning faithfulness for three GLLMs across increasing cognitive complexities, using PCC. 
    A stronger negative correlation indicates a better uncertainty metric.
    %\textit{Results}: 
    Baselines exhibit strong but regime-specific performance, whereas GRCS yields the strongest negative correlation in 8 of the 15 configurations and remains consistently negative in 14 out of 15 (93\%), establishing it as the most reliable indicator across scales.}\label{fig:gsm8k_res}
    \vspace{-5mm}
\end{wrapfigure}
%\end{figure}

==> pic/rq3_1_pics.tex <==
\begin{figure*}[t]
\centering
\setlength{\tabcolsep}{3pt}

% ==========================================
% STRATEGYQA PLOTS
% ==========================================
% Row 1: scatter plot + DeepSeek KDE
\begin{minipage}[t]{0.45\textwidth}
    \centering
    \textbf{(a) StrategyQA: Reasoning topology}\par\vspace{0.1em}
    \includegraphics[width=0.70\linewidth]{pic/strategyqa_quadrants.pdf}
\end{minipage}
\hfill
\begin{minipage}[t]{0.45\textwidth}
    \centering
    \textbf{(b) StrategyQA: DeepSeek R1 KDE}\par\vspace{0.05em}
    \begin{subfigure}[t]{\linewidth}
        \centering
        \includegraphics[width=0.70\linewidth]{pic/strategyqa_kde_deepseek.pdf}
        \phantomcaption
        \label{fig:strategyqa_deepseek_kde}
    \end{subfigure}
\end{minipage}
\vspace{0.2em}

% Row 2: Phi-4 KDE + Llama KDE
\begin{minipage}[t]{0.45\textwidth}
    \centering
    \textbf{(c) StrategyQA: Phi-4 KDE}\par\vspace{0.05em}
    \includegraphics[width=0.70\linewidth]{pic/strategyqa_kde_phi4.pdf}
\end{minipage}
\hfill
\begin{minipage}[t]{0.45\textwidth}
    \centering
    \textbf{(d) StrategyQA: Llama-3.1-8B KDE}\par\vspace{0.05em}
    \includegraphics[width=0.70\linewidth]{pic/strategyqa_kde_Llama.pdf}
\end{minipage}

\vspace{1.5em} % Adds vertical space between the two datasets
\hrule % Optional: adds a subtle line to separate the datasets
\vspace{1.5em}

% ==========================================
% GPQA PLOTS
% ==========================================
% Row 3: scatter plot + DeepSeek KDE
\begin{minipage}[t]{0.45\textwidth}
    \centering
    \textbf{(e) GPQA: Reasoning topology}\par\vspace{0.1em}
    \includegraphics[width=0.70\linewidth]{pic/gpqa_quadrants.pdf}
\end{minipage}
\hfill
\begin{minipage}[t]{0.45\textwidth}
    \centering
    \textbf{(f) GPQA: DeepSeek R1 KDE}\par\vspace{0.05em}
    \begin{subfigure}[t]{\linewidth}
        \centering
        \includegraphics[width=0.70\linewidth]{pic/gpqa_kde_deepseek.pdf}
        \phantomcaption
        \label{fig:gpqa_deepseek_kde}
    \end{subfigure}
\end{minipage}
\vspace{0.2em}

% Row 4: Phi-4 KDE + Llama KDE
\begin{minipage}[t]{0.45\textwidth}
    \centering
    \textbf{(g) GPQA: Phi-4 KDE}\par\vspace{0.05em}
    \includegraphics[width=0.70\linewidth]{pic/gpqa_kde_phi4.pdf}
\end{minipage}
\hfill
\begin{minipage}[t]{0.45\textwidth}
    \centering
    \textbf{(h) GPQA: Llama-3.1-8B KDE}\par\vspace{0.05em}
    \includegraphics[width=0.70\linewidth]{pic/gpqa_kde_Llama.pdf}
\end{minipage}

\caption{\textbf{Reasoning topology on StrategyQA and GPQA in the $(\text{Divergence}, \text{Entropy})$ space.}
Each question $q$ is plotted by its mean Divergence ($x$; coherence) and Entropy ($y$; heterogeneity) across $N=20$ paths. 
\textbf{(a--d) StrategyQA:} Anchored by the Llama 3.1 8B mean as the reference center, DeepSeek R1 exhibits the broadest, highest-entropy exploration, while Llama 3.1 8B and Phi-4 cluster tightly at lower entropy levels. 
\textbf{(e--h) GPQA:} Overall entropy drops across all models on this harder dataset, but the relative ordering is preserved. DeepSeek R1 consistently sustains the highest diversity into the \emph{Multi-Path} and \emph{Confused} quadrants, Phi-4 acts as a middle ground, and Llama 3.1 8B collapses almost entirely into the low-variance \emph{Confident} regime.
}
\label{fig:combined_reasoning_topology_appendix}
\end{figure*}

==> pic/topology_gpqa.tex <==
\begin{figure*}[t]
\centering
\setlength{\tabcolsep}{3pt}
% Row 1: scatter plot + DeepSeek KDE
\begin{minipage}[t]{0.45\textwidth}
    \centering
    \textbf{(a) Reasoning topology across models}\par\vspace{0.1em}
    \includegraphics[width=0.70\linewidth]{pic/gpqa_quadrants.pdf}
\end{minipage}
\hfill
\begin{minipage}[t]{0.45\textwidth}
    \centering
    \textbf{(b) DeepSeek R1 KDE}\par\vspace{0.05em}
    \begin{subfigure}[t]{\linewidth}
        \centering
        \includegraphics[width=0.70\linewidth]{pic/gpqa_kde_deepseek.pdf}
        \phantomcaption
        \label{fig:deepseek_kde}
    \end{subfigure}
\end{minipage}
\vspace{0.2em}

% Row 2: Phi-4 KDE + Llama KDE
\begin{minipage}[t]{0.45\textwidth}
    \centering
    \textbf{(c) Phi-4 KDE}\par\vspace{0.05em}
    \includegraphics[width=0.70\linewidth]{pic/gpqa_kde_phi4.pdf}
\end{minipage}
\hfill
\begin{minipage}[t]{0.45\textwidth}
    \centering
    \textbf{(d) Llama-3.1-8B KDE}\par\vspace{0.05em}
    \includegraphics[width=0.70\linewidth]{pic/gpqa_kde_Llama.pdf}
\end{minipage}

\caption{\textbf{Reasoning topology on StrategyQA in the $(\text{Divergence}, \text{Entropy})$ space.}
Each question $q$ is plotted by its mean Divergence ($x$; coherence) and Entropy ($y$; heterogeneity) across $N=20$ paths. \textbf{(a)} Llama 3.1 8B mean ($\mu=(0.31, 0.85)$) is taken as reference center, defining four regimes: \emph{Confident}, \emph{Multi-Path}, \emph{Noisy}, \emph{Confused}. DeepSeek R1 ($\mu=(0.325, 1.032)$) spans the broadest, highest-entropy region---diffuse exploration across \emph{Multi-Path} and \emph{Confused}. Llama 3.1 8B and Phi-4 ($\mu=(0.301, 0.748)$) cluster tightly at lower entropy, reflecting stronger mode collapse and more rigid reasoning. \textbf{(b--d)} KDE density plots for each model individually: DeepSeek R1 peaks at $(0.376, 1.207)$, Phi-4 at $(0.289, 0.718)$, and Llama 3.1 8B at $(0.287, 0.947)$, confirming DeepSeek R1's markedly higher entropy and divergence relative to both smaller models.
%\fixme{The axis labels are not still readable.}
%\rreva{also, here put meda/gpqa plots as well}
}
\label{fig:reasoning_topology_gpqa}
\end{figure*}

==> pic/uq_analysis_minipage.tex <==
\begin{figure*}
    \centering
    %\includegraphics[width=0.65\textwidth]
    \includegraphics[scale=0.17]
    {pic/uq_bars_PCC_new.pdf}
    \caption{\textbf{UQ Analysis}. 
    %\textit{Methodology}: We measure how well different uncertainty metrics correlate with actual reasoning Faithfulness across three LLMs on GSM8K dataset, reporting Pearson (PCC), Spearman (SRC) and Kendall (KRC) correlations. A reliable uncertainty metric must show a strong negative correlation with Faithfulness. 
    %\textit{Methodology}: We correlate uncertainty with reasoning faithfulness for three GLLMs across increasing cognitive complexities, using PCC. 
    A stronger negative correlation indicates a better uncertainty metric.
    %\textit{Results}: 
    Baselines exhibit strong but regime-specific performance, whereas GRCS yields the strongest negative correlation in 8 of the 15 configurations and remains negatively
    correlated with faithfulness
    %consistently negative 
    in 14 out of 15 (93\%), establishing it as the most reliable indicator across scales.}
    \label{fig:gsm8k_res}
    \vspace{-6mm}
\end{figure*}

==> src/ethics.tex <==
\section{Ethics Statement}

This work uses public benchmark data and model-generated reasoning traces, without human subjects or private information. We do not identify direct ethical concerns specific to our experimental setting, beyond the broader risks associated with the use of LLMs.

==> src/unneded.tex <==
\noindent {\bf Graph Self-Consistency (GSC)}.
\begin{comment}
While standard
SC selects the most reliable answer through a majority voting scheme on the output paths %outputs 
\citep{wang2023selfconsistency}, it ignores the logical validity of the intermediate steps, raising a serious concern: %. The problem is, 
if we are %want 
to trust LLMs in safety-critical applications, we must eliminate \emph{lucky guesses} and post-hoc hallucinations. An answer can only be considered truly reliable if we first rigorously analyze and verify the reasoning process that produced it. To address this, we introduce Graph Self-Consistency (GSC), a selection-based approach that identifies the most representative and logically sound reasoning path from the generated pool. By evaluating the reasoning space topologically, Graph-SC selects the \emph{medoid CoT}. The medoid represents the structural and semantic center of the model's reasoning space.  To ensure the selected CoT is both structurally central and semantically verified, we compute a combined selection score that is formed by two components: Structural Centrality and Path Consensus.

We build a pairwise SS-GED matrix and %then we 
calculate the similarity between all generated CoTs. For a given question, let $S(G_i, G_j) = 1 - d(G_i, G_j)$ represent the similarity between graphs $G_i$ and $G_j$. The Structural Centrality $C(G_i)$ of a CoT is the sum of its similarities to all other generated reasoning paths:
$
    C(G_i) = \sum_{j \neq i} S(G_i, G_j)
$
Graphs with high centrality represent the dominant reasoning topology utilized by the LLM. To penalize reasoning paths that contain isolated hallucinations, we introduce a fine-grained Node Consensus score. For every node $v$ in a graph $G_i$, we calculate the fraction of other generated graphs that contain at least one node with a highly similar semantic embedding (cosine similarity $\ge 0.9$). 
We then aggregate these node scores to compute the Path Consensus score $P(G_i)$ for the entire CoT. Because hallucinated conclusions are catastrophic to accuracy, terminal nodes (nodes with an out-degree of $0$) are assigned a higher multiplier weight of $2.0$ during this aggregation.
The final Medoid CoT is selected by maximizing the weighted combination of normalized Structural Centrality and Semantic Path Consensus:
$
    \text{Medoid} = \arg\max_{G_i} \left[ \alpha \frac{C(G_i)}{\max_j C(G_j)} + (1 - \alpha) P(G_i) \right]
$
In our experiments, we set $\alpha = 0.8$,  
prioritizing structural consensus while allowing Path Consensus to break ties and filter out CoTs with unsupported terminal conclusions. We found the framework to be qualitatively stable across nearby values of $\alpha$. The final answer associated with this Medoid CoT is extracted and considered the framework's final prediction. %, ensuring high-fidelity reasoning.
\end{comment}

==> tables/ablation_table.tex <==
\begin{table}[H]
\begin{center}
\small
\begin{tabular}{llrcccc}
\toprule
\multicolumn{1}{c}{\bf Dataset} &
\multicolumn{1}{c}{\bf Model} &
\multicolumn{1}{c}{\bf N} &
\multicolumn{1}{c}{\bf AA} &
\multicolumn{1}{c}{\bf AF} &
\multicolumn{1}{c}{\bf OF} &
\multicolumn{1}{c}{\bf MD} \\
\midrule
GSM8K   & Llama 3.1 8B   & 16 & 0.000          & \textbf{1.000} & 0.510          & 0.576          \\
GSM8K   & Phi-4          & 14 & 0.000          & \textbf{1.000} & \textbf{0.597} & 0.712          \\
GSM8K   & DeepSeek R1    &  7 & 0.000          & 0.857          & 0.551          & \textbf{0.784} \\
\midrule
BoolQ   & Llama 3.1 8B   &  9 & 0.559          & 0.530          & \textbf{0.542} & 0.769          \\
BoolQ   & Phi-4          &  7 & 0.438          & 0.459          & 0.264          & 0.681          \\
BoolQ   & DeepSeek R1    &  3 & 0.333          & \textbf{0.705} & 0.274          & \textbf{0.838} \\
\midrule
StratQA & Llama 3.1 8B   &  5 & 0.507          & 0.364          & \textbf{0.657} & 0.745          \\
StratQA & Phi-4          &  8 & 0.500          & 0.499          & 0.402          & 0.778          \\
StratQA & DeepSeek R1    &  5 & 0.387          & \textbf{0.597} & 0.153          & \textbf{0.935} \\
\midrule
MedQA   & Llama 3.1 8B   &  1 & 0.700          & \textbf{0.874} & \textbf{0.769} & 0.681          \\
MedQA   & Phi-4          &  3 & 0.678          & 0.543          & 0.484          & 0.693          \\
MedQA   & DeepSeek R1    &  1 & \textbf{1.000} & 0.000          & 0.333          & \textbf{0.995} \\
\midrule
GPQA    & Llama 3.1 8B   & 16 & 0.438          & \textbf{0.614} & \textbf{0.556} & \textbf{0.758} \\
GPQA    & Phi-4          & 14 & 0.462          & 0.472          & 0.522          & 0.712          \\
GPQA    & DeepSeek R1    &  6 & 0.500          & 0.333          & 0.551          & 0.751          \\   
\bottomrule
\end{tabular}
\end{center}
\caption{Results per dataset and model. Bold denotes the best value per dataset block. Alt.\ = alternative (adversarial); Faith.\ = faithfulness; Medoid Dist.\ = average medoid distance.}
\label{table:target_abl_table_results_appendix}
\end{table}

==> tables/aime_arxiv.tex <==
\vspace{3mm}
\begin{table}[htbp]
\centering
\caption{Pearson Correlation Coefficient (PCC) between Faithfulness and various uncertainty metrics on the AIME-2026 dataset.}
\label{tab:aime_evaluation}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccc}
\toprule
\textbf{GLLM} & \textbf{PCC - GRCS (ours)} & \textbf{PCC - Topo-UQ} & \textbf{PCC - CoTA} & \textbf{PCC - Dispersion} & \textbf{PCC - Entropy} \\
\midrule
Llama 3.1 & 0.04 & 0.16 & 0.05 & \textbf{-0.22} & \textbf{-0.22} \\
Phi-4 & \textbf{-0.25} & 0.07 & 0.01 & 0.08 & 0.10 \\
DeepSeek R1 & \textbf{-0.54} & 0.25 & 0.12 & -0.05 & -0.24 \\
\bottomrule
\end{tabular}
}
\end{table}
\vspace{3mm}

==> tables/counterfactuals_pearl.tex <==
\vspace{3mm}
\begin{table}[htbp]
\centering
\caption{Comparison of Pearson Correlation Coefficients using Early Answering (PCC-EA) and Counterfactual Editing (PCC-CF) as faithfulness measures.}
\label{tab:counterfactual_editing}
\resizebox{\textwidth}{!}{
\begin{tabular}{llccc}
\toprule
\textbf{Dataset} & \textbf{GLLM} & \textbf{PCC-EA} & \textbf{PCC-CF} & $\boldsymbol{\Delta(\text{CF} - \text{EA})}$ \\
\midrule
GPQA & Llama 3.1 & 0.006 & -0.004 & -0.010 \\
GPQA & Phi-4 & -0.109 & -0.129 & -0.020 \\
GPQA & DeepSeek R1 & -0.023 & -0.0198 & +0.003 \\
\midrule
MedQA & Llama 3.1 & -0.280 & -0.320 & -0.040 \\
MedQA & Phi-4 & -0.240 & -0.233 & +0.007 \\
MedQA & DeepSeek R1 & -0.105 & -0.111 & -0.006 \\
\midrule
StrategyQA & Llama 3.1 & -0.210 & -0.101 & +0.109 \\
StrategyQA & Phi-4 & -0.071 & -0.233 & -0.162 \\
StrategyQA & DeepSeek R1 & -0.182 & -0.240 & -0.058 \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/datasets.tex <==
\begin{table}[ht]
\centering
\caption{Evaluation datasets. We select four benchmarks spanning
commonsense, scientific, clinical, and mathematical reasoning,
covering a spectrum from general-purpose to more critical domains
and from moderate to expert-level difficulty.}
\label{tab:datasets}
\begin{tabular}{lllp{5.8cm}}
\toprule
\textbf{Dataset} & \textbf{Split} & \textbf{Size} & \textbf{Rationale} \\
\midrule
GPQA Diamond \citep{rein2024gpqa}
  & Test & 198
  & Graduate-level science (biology, chemistry, physics).
    Expert-level multi-step causal reasoning; our primary showcase
    dataset. No prior UQ framework evaluates on this benchmark. Fully test set used without subsampling.\\
\addlinespace
StrategyQA \citep{geva2021aristotle}
  & Dev & 229
  & Commonsense multi-hop boolean reasoning.
    Full dev set used without subsampling.
    Contrasts GPQA Diamond: open-domain, shorter reasoning chains. \\
\addlinespace
MedQA USMLE \citep{jin2021whatdisease}
  & Test & 100$^\dagger$
  & Clinical multi-step reasoning
    (symptom $\to$ mechanism $\to$ diagnosis $\to$ treatment).
    Grounds the framework in a high-stakes domain where reasoning
    determinism is safety-critical; motivates the aleatoric
    vs.\ epistemic uncertainty analysis. \\
\addlinespace
GSM8K \citep{cobbe2021training}
  & Test & 100$^\dagger$
  & Grade-school arithmetic word problems.
    Included to enable methodological comparison with
    Topo-UQ \citep{da2025understanding}, which also evaluates on GSM8K.
    Structured numerical graphs provide a controlled contrast
    to the open-ended causal graphs of GPQA and StrategyQA. \\
\bottomrule
\end{tabular}
\begin{minipage}{\linewidth}
\small $^\dagger$ Randomly subsampled with seed 42 for computational
feasibility (MedQA test = 1{,}273; GSM8K test = 1{,}319).
\end{minipage}
\end{table}

==> tables/dllms_ablation_1.tex <==
\begin{table}[htbp]
\centering
\caption{Decomposition Quality across different Decomposer LLMs.}
\label{tab:dllm_quality}
\begin{tabular}{lccc}
\toprule
\textbf{DLLM} & \textbf{Atomicity} & \textbf{Absence of Hallucination} & \textbf{Dependency Validity} \\
\midrule
GPT-4o & 94.2\% & 95.6\% & 74.1\% \\
Mistral-Large-2512 & 97.8\% & 95.8\% & 77.0\% \\
GPT-OSS-120b & 88.0\% & 97.5\% & 73.5\% \\
Gemini 3 Flash & 98.7\% & 96.0\% & 68.8\% \\
\bottomrule
\end{tabular}
\end{table}

==> tables/dllms_ablation_2.tex <==
\vspace{1mm}
\begin{table}[htbp]
\centering
\caption{Inter-DLLM agreement study on graph dimensions across datasets.}
\label{tab:dllm_agreement}
\begin{tabular}{llcc}
\toprule
\textbf{Dataset} & \textbf{Decomposer LLM} & \textbf{Avg Fact Nodes per CoT} & \textbf{Avg Edges per Fact} \\
\midrule
GPQA & GPT-4o & 24.29 & 0.83 \\
GPQA & Mistral-Large-2512 & 22.30 & 1.01 \\
GPQA & GPT-OSS-120b & 15.27 & 0.99 \\
GPQA & Gemini 3 Flash & 19.00 & 0.91 \\
\midrule
MedQA & GPT-4o & 14.24 & 0.77 \\
MedQA & Mistral-Large-2512 & 17.31 & 0.90 \\
MedQA & GPT-OSS-120b & 14.18 & 0.88 \\
MedQA & Gemini 3 Flash & 15.95 & 0.94 \\
\midrule
StrategyQA & GPT-4o & 10.45 & 0.80 \\
StrategyQA & Mistral-Large-2512 & 9.84 & 0.84 \\
StrategyQA & GPT-OSS-120b & 7.96 & 0.83 \\
StrategyQA & Gemini 3 Flash & 9.20 & 0.82 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/dllms_ablation_3.tex <==
\vspace{3mm}
\begin{table}[htbp]
\centering
\caption{Pearson Correlation Coefficient (PCC) of alternative DLLMs with respect to the baseline GPT-4o.}
\label{tab:dllm_pcc}
\begin{tabular}{llc}
\toprule
\textbf{Dataset} & \textbf{Decomposer LLM} & \textbf{PCC wrt GPT-4o} \\
\midrule
GPQA & Mistral-Large-2512 & 0.77 \\
GPQA & GPT-OSS-120b & 0.73 \\
GPQA & Gemini 3 Flash & 0.72 \\
\midrule
MedQA & Mistral-Large-2512 & 0.86 \\
MedQA & GPT-OSS-120b & 0.87 \\
MedQA & Gemini 3 Flash & 0.94 (highest) \\
\midrule
StrategyQA & Mistral-Large-2512 & 0.66 \\
StrategyQA & GPT-OSS-120b & 0.57 (lowest) \\
StrategyQA & Gemini 3 Flash & 0.74 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/jidall.tex <==
\begin{table}
\centering
\small
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{l l l c}
\toprule
\textbf{CoT} & \textbf{Hallucinated school} & \textbf{Hallucinated mascot} & \textbf{GLLM Final Answer} \\
\midrule
CoT 2  & Louisiana generic   & Alligator                         & false \\
CoT 3  & \textbf{Baton Rouge High} & Tiger                 & false \\
CoT 5  & \textbf{Baton Rouge High} & Panthers                       & false \\
CoT 9  & \textbf{Baton Rouge Magnet}  & Panthers                          & false \\
CoT 11 & Louisiana generic   & Wildcats                          & false \\
CoT 12 & Unknown             & Tiger / Eagle                     & false \\
CoT 14 & Louisiana generic   & Unknown                           & false \\
CoT 15 & Unknown                 & Symbol, not animal                & false \\
CoT 18 & Catholic school     & Saints                            & false \\
CoT 19 & \textbf{Baton Rouge Magnet}  & Tigers                            & false \\
CoT 20 & \textbf{Baton Rouge Magnet}  & Eagles                            & false \\
CoT 4  & \textbf{Baton Rouge High} & \textbf{Bulldog} $\rightarrow$ but mascot is a symbol & false \\
\bottomrule
\end{tabular}
\caption{Incorrect \emph{false} CoTs and their hallucinated intermediate facts. The correct school and mascot, when mentioned, are highlighted in bold. Even when the correct pair is partially recovered, the reasoning may still derail, illustrating the internal inconsistency of the \emph{false} cluster.}
\label{tab:no_cot_fragmentation_jindall}
\end{table}

==> tables/longer_traces.tex <==
\begin{table}[htbp]
\centering
\caption{Comparison of average GED and SS-GED between Baseline (3--6 steps) and Extended (10--20 steps) reasoning traces.}
\label{tab:scalability_ged}
\resizebox{\textwidth}{!}{
\begin{tabular}{llcccc}
\toprule
\textbf{Dataset} & \textbf{GLLM} & \textbf{Avg GED - Baseline} & \textbf{Avg GED - Extended} & \textbf{Avg SS-GED - Baseline} & \textbf{Avg SS-GED - Extended} \\
\midrule
GPQA & Llama 3.1 & 5.19 & 9.69 (1.87x) & 0.09 & 0.09 (Stable) \\
GPQA & Phi-4 & 4.92 & 8.57 (1.74x) & 0.32 & 0.35 (Stable) \\
GPQA & DeepSeek R1 & 3.02 & 10.11 (3.35x) & 0.34 & 0.23 (Stable) \\
\midrule
MedQA & Llama 3.1 & 7.22 & 16.23 (2.25x) & 0.33 & 0.40 (Stable) \\
MedQA & Phi-4 & 13.50 & 25.10 (1.86x) & 0.32 & 0.32 (Stable) \\
MedQA & DeepSeek R1 & 5.69 & 11.55 (2.03x) & 0.30 & 0.29 (Stable) \\
\midrule
StratQA & Llama 3.1 & 6.72 & 12.97 (1.93x) & 0.32 & 0.34 (Stable) \\
StratQA & Phi-4 & 7.03 & 14.22 (2x) & 0.30 & 0.32 (Stable) \\
StratQA & DeepSeek R1 & 4.17 & 10.11 (2.42x) & 0.34 & 0.23 (Stable) \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/notations.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{c|c}
        \hline
        {\bf Acronym/Notation} &  {\bf Explanation}\\
        \hline\hline
         LLM & Large-Language Model \\ 
         CoT & Chain of thought \\
         UQ & Uncertainty Quantification \\ 
         SC & Self Consistency \\
         GRCS & Graph Reasoning Coherence Score \\ 
         GSC & Graph Self Consistency \\ 
         GED & Graph Edit Distance \\
         SS-GED & Structural-Semantic Graph Edit Distance \\
         GLLM & Generator LLM \\
         DLLM & Decomposer LLM \\ 
         RBF & Radial Basis Function \\ 
         $q$ & A question \\
         $\mathfrak{D}(q)$ & Pairwise distance set \\
         ${\cal D}(q)$ & Divergence \\
         ${\cal C}(q)$ & Convergence \\
         $\sigma_{\mathfrak{D}(q)}$ & Dispersion \\ 
         $H{(\mathfrak{D}(q))}$ & Entropy \\   
         $G = (V, E)$ & Causal dependency graph \\
         $\beta$ & Semantic similarity weight \\
         $\gamma$ &  RBF Controller\\
         $\alpha$ & trade-off between centrality and support\\
         $C(G_i)$ & Structural centrality \\
         $P(G_i)$ & Graph-level consensus score\\
         $z^\star$ & medoid CoT\\
         $x_q$ & Original GLLM prompt\\
         $z^\star_q$ & medoid CoT selected by GSC\\
         $\delta_{ablate}$ & Adversartial perturbation \\
         $x^\prime$ & Poisoned prompt\\
         \hline
    \end{tabular}
    \caption{Notations and Acronyms used in this work.}
    \label{table:notations}    
\end{table}

==> tables/ss_ged_sensitivity2.tex <==
\begin{table}[htbp]
\centering
\caption{$\gamma$ sensitivity with $\beta=0.4$ fixed. Each cell reports PCC / GSC accuracy.}
\label{tab:gamma_sensitivity}
\resizebox{\textwidth}{!}{
\begin{tabular}{llcccccc}
\toprule
\textbf{Dataset} & \textbf{Model} & $\boldsymbol{\gamma=0.5}$ & $\boldsymbol{\gamma=1}$ & $\boldsymbol{\gamma=2.5}$ & $\boldsymbol{\gamma=5}$ & $\boldsymbol{\gamma=10}$ & $\boldsymbol{\gamma=20}$ \\
\midrule
GPQA & Llama 3.1 & 0.012 / 19.3\% & -0.003 / 17.3\% & 0.012 / 15.3\% & 0.006 / 19.3\% & 0.057 / 19.3\% & 0.031 / 17.3\% \\
GPQA & Phi-4 & -0.059 / 28.8\% & -0.090 / 32.8\% & -0.076 / 32.8\% & -0.100 / 32.8\% & -0.049 / 30.8\% & -0.013 / 32.8\% \\
GPQA & DeepSeek R1 & -0.052 / 53.4\% & -0.018 / 53.4\% & -0.027 / 53.4\% & -0.020 / 53.4\% & -0.101 / 53.4\% & -0.122 / 53.4\% \\
\midrule
MedQA & Llama 3.1 & -0.278 / 52.0\% & -0.266 / 52.0\% & -0.270 / 52.0\% & -0.280 / 52.0\% & -0.269 / 54.0\% & -0.250 / 52.0\% \\
MedQA & Phi-4 & -0.262 / 77.0\% & -0.245 / 79.0\% & -0.232 / 79.0\% & -0.240 / 79.0\% & -0.234 / 77.0\% & -0.286 / 77.0\% \\
MedQA & DeepSeek R1 & -0.142 / 91.9\% & -0.108 / 91.9\% & -0.117 / 91.9\% & -0.110 / 91.9\% & -0.191 / 91.9\% & -0.212 / 91.9\% \\
\midrule
StrategyQA & Llama 3.1 & -0.208 / 71.6\% & -0.196 / 71.6\% & -0.200 / 71.6\% & -0.210 / 71.6\% & -0.199 / 73.6\% & -0.180 / 71.6\% \\
StrategyQA & Phi-4 & -0.092 / 74.7\% & -0.075 / 76.7\% & -0.062 / 76.7\% & -0.070 / 76.7\% & -0.064 / 74.7\% & -0.116 / 74.7\% \\
StrategyQA & DeepSeek R1 & -0.212 / 78.2\% & -0.178 / 78.2\% & -0.187 / 78.2\% & -0.180 / 78.2\% & -0.261 / 78.2\% & -0.282 / 78.2\% \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/ss_gedsensitivity.tex <==
\begin{table}[htbp]
\centering
\caption{$\beta$ sensitivity with $\gamma=5.0$ fixed. Each cell reports PCC / GSC accuracy.}
\label{tab:beta_sensitivity}
\resizebox{\textwidth}{!}{
\begin{tabular}{llcccccc}
\toprule
\textbf{Dataset} & \textbf{Model} & $\boldsymbol{\beta=0.0}$ & $\boldsymbol{\beta=0.2}$ & $\boldsymbol{\beta=0.4}$ & $\boldsymbol{\beta=0.6}$ & $\boldsymbol{\beta=0.8}$ & $\boldsymbol{\beta=1.0}$ \\
\midrule
GPQA & Llama 3.1 & 0.043 / 20.7\% & 0.020 / 17.3\% & 0.006 / 19.3\% & 0.021 / 19.3\% & -0.010 / 23.3\% & -0.042 / 20.7\% \\
GPQA & Phi-4 & -0.122 / 31.8\% & -0.059 / 36.8\% & -0.100 / 32.8\% & -0.053 / 32.8\% & -0.077 / 32.8\% & -0.054 / 27.9\% \\
GPQA & DeepSeek-R1 & -0.009 / 51.8\% & -0.017 / 53.4\% & -0.020 / 53.4\% & -0.060 / 53.4\% & -0.049 / 53.4\% & -0.038 / 51.8\% \\
\midrule
MedQA & Llama 3.1 & -0.262 / 52.4\% & -0.273 / 54.0\% & -0.280 / 52.0\% & -0.266 / 52.0\% & -0.257 / 52.0\% & -0.273 / 50.4\% \\
MedQA & Phi-4 & -0.258 / 74.7\% & -0.231 / 79.0\% & -0.240 / 79.0\% & -0.246 / 79.0\% & -0.248 / 77.0\% & -0.242 / 74.7\% \\
MedQA & DeepSeek-R1 & -0.096 / 89.1\% & -0.107 / 91.9\% & -0.110 / 91.9\% & -0.150 / 91.9\% & -0.139 / 91.9\% & -0.126 / 89.1\% \\
\midrule
StrategyQA & Llama 3.1 & -0.194 / 71.4\% & -0.203 / 73.6\% & -0.210 / 71.6\% & -0.196 / 71.6\% & -0.187 / 71.6\% & -0.205 / 69.5\% \\
StrategyQA & Phi-4 & -0.093 / 72.5\% & -0.061 / 76.7\% & -0.070 / 76.7\% & -0.076 / 76.7\% & -0.078 / 74.7\% & -0.077 / 72.5\% \\
StrategyQA & DeepSeek-R1 & -0.164 / 75.9\% & -0.177 / 78.2\% & -0.180 / 78.2\% & -0.220 / 78.2\% & -0.209 / 78.2\% & -0.194 / 75.9\% \\
\bottomrule
\end{tabular}
}
\end{table}
